Supervising the Multi-Fidelity Race of Hyperparameter Configurations

Multi-fidelity (gray-box) hyperparameter optimization techniques (HPO) have recently emerged as a promising direction for tuning Deep Learning methods. However, existing methods suffer from a sub-optimal allocation of the HPO budget to the hyperparameter configurations. In this work, we introduce DyHPO, a Bayesian Optimization method that learns to decide which hyperparameter configuration to train further in a dynamic race among all feasible configurations. We propose a new deep kernel for Gaussian Processes that embeds the learning curve dynamics, and an acquisition function that incorporates multi-budget information. We demonstrate the significant superiority of DyHPO against state-of-the-art hyperparameter optimization methods through large-scale experiments comprising 50 datasets (Tabular, Image, NLP) and diverse architectures (MLP, CNN/NAS, RNN).

==> Text/2_motivation.tex <==
\section{Motivation} 

As mentioned earlier, a major source of sub-optimality for the current gray-box techniques~\citep{Li2017,Falkner2018,Awad2021} is the poor rank correlation of performances at low and high budgets, which is endemic to the successive halving mechanism. In essence, prior methods mistakenly discard good hyper-parameter configurations by myopically relying only on the early performance after a few epochs, following a fixed fidelity scheme. In contrast, our method uses a dynamic fidelity allocation scheme that tackles the endemic poor correlation of successive halving, by learning to decide which configuration to continue optimizing for one more time-budget step (e.g. one more epoch). In that perspective, our strategy resembles Freeze-Thaw~\citep{Swersky2014}, however, differs in fitting deep kernel GP surrogates with learning curves and a tailored multi-budget acquisition. \algabbr{} never discards a configuration as all options remain latent until the acquisition selects the most promising one and allocates one more budget unit of optimization. 


We illustrate the differences between our strategy and successive halving with the experiment of Figure~\ref{fig:motivation}, where we showcase the HPO progress of two different methods on the "Helena" dataset from the LCBench benchmark~\citep{Zimmer2021}.
%Random search is an example of a black-box approach that trains each candidate until completion without considering the intermediate scores.
Hyperband~\citep{Li2017} is a gray-box approach that \textit{statically} pre-allocates the budget for a set of candidates (Hyperband bracket) according to a predefined policy.
However, \algabbr{} \textit{dynamically} adapts the allocation of budgets for configurations after every HPO step.

The plots in the top row of Figure~\ref{fig:motivation} show the learning curves of multiple neural networks trained with different hyperparameter configurations.
The darker the color of a learning curve, the later the model corresponding to the learning curve was trained during the optimization process.
In an optimal scenario, there should be no learning curve of darker color trained for a very long time if there is already a learning curve of lighter color with higher accuracy.
In black-box functions, this trend would not be observed as intermediate responses are not considered.
However, it is also not the case for gray-box methods such as Hyperband, because it is possible that no configuration selected for a Hyperband bracket is outperforming the current best configuration.
Since at least one of the bracket candidates must be fully trained according to the predefined policy, we observe this suboptimal behavior in Figure~\ref{fig:motivation}.
This motivates our idea of dynamically deciding when we want to continue training a configuration based on the intermediate response.
Clearly, as observed in Figure~\ref{fig:motivation}, \algabbr{} invests only a small budget into configurations that show little promise as indicated by the intermediate scores.

==> Text/2_old_motivation.tex <==
\section{Motivation} 

As mentioned earlier, a major source of sub-optimality for the current gray-box techniques~\citep{Li2017,Falkner2018,Awad2021} is the poor rank correlation of performances at low and high budgets, which is endemic to the successive halving mechanism. In essence, prior methods mistakenly discard good hyper-parameter configurations by myopically relying only on the early performance after few epochs. In contrast, our method fixes the endemic poor correlation of successive halving, by learning to decide which configuration to continue optimizing for one more time-budget step (e.g. one more epoch). In that perspective, our strategy resembles Freeze-Thaw~\citep{Swersky2014}, however, differs in fitting deep kernel GP surrogates with learning curves and a special multi-budget acquisition. \algabbr{} never discards a configuration as all options remain latent until the acquisition selects the most promising one and allocates one more budget unit of optimization. 

\begin{figure}[t]
  \centering
  \includegraphics[width=1\columnwidth]{fig/motivation.pdf}
  \caption{Top row: Learning curves observed during the search. The darker the learning curve, the later it was evaluated during the search.
        Bottom row: y-axis shows a sequence of learning curve evaluations (bottom to top). The color indicates accuracy. The darker red the higher the accuracy.}
  \label{fig:motivation}
\end{figure}

We illustrate the differences between our strategy and successive halving with the experiment of Figure~\ref{fig:motivation}, where we showcase the HPO progress of three different methods on the "Helena" dataset from the LCBench benchmark~\citep{Zimmer2021}.
%Random search is an example of a black-box approach that trains each candidate until completion without considering the intermediate scores.
Hyperband~\citep{Li2017} is a gray-box approach that \textit{statically} pre-allocates the budget for a set of candidates (Hyperband bracket) according to a predefined policy.
However, \algabbr{} \textit{dynamically} adapts the allocation of budgets for configurations after every HPO step.

The plots in the top row of Figure~\ref{fig:motivation} show the learning curves of multiple neural networks trained with different hyperparameter configurations.
The darker the color of a learning curve, the later the model corresponding to the learning curve was trained during the optimization process.
In an optimal scenario, there should be no learning curve of darker color trained for a very long time if there is already a learning curve of lighter color with higher accuracy.
Since black-box functions do not consider intermediate responses, this trend would not be observed.
However, it is also not the case for gray-box methods such as Hyperband, because it is possible that no configuration selected for a Hyperband bracket is outperforming the current best configuration.
Since at least one of the bracket candidates must be fully trained according to the predefined policy, we observe this suboptimal behavior in Figure~\ref{fig:motivation}.
This motivates our idea of dynamically deciding when we want to continue training a configuration based on the intermediate response.
Clearly, \algabbr{} invests only a small budget into configurations that show little promise as indicated by the intermediate scores.

==> Text/3_old_related_work.tex <==
\section{Related Work on Gray-box HPO}
\paragraph*{Multi-Fidelity Bayesian Optimization and Bandits.}
Bayesian optimization is a black-box function optimization framework that has been successfully applied in optimizing hyperparameter and neural architectures alike~\citep{Snoek2012,Kandasamy2018, Bergstra2011}.
To further improve Bayesian optimization, several works propose low-fidelity data approximations of hyperparameter configurations.
Low-fidelity approximations of hyperparameter configurations can be obtained by training on a subset of the data~\citep{Swersky2013, Klein2017} or terminating training early~\citep{Swersky2014}.
Several methods extend Bayesian optimization to multi-fidelity data by engineering new kernels suited for this problem~\citep{Swersky2013,Swersky2014,Poloczek2017}.
\cite{Kandasamy2016} extends GP-UCB~\citep{Srinivas2010} to the multi-fidelity setting by learning one Gaussian Process (GP) with a standard kernel for each fidelity.
Their later work improves upon this method by learning one GP for all fidelities that enables the use of continuous fidelities~\citep{Kandasamy2017}.
The work by \cite{Takeno2020} follows a similar idea but proposes to use an acquisition function based on information gain instead of UCB.
While most of the works rely on GPs to model the surrogate function, \cite{Li2020} use a Bayesian neural network that models the complex relationship between fidelities with stacked neural networks, one for each fidelity.

% Previous implementation
% \paragraph*{Multi-Fidelity Bandits and Bayesian Optimization}
%Hyperband~\citep{Li2017} is a multi-fidelity method for hyperparameter optimization which, due to its simplicity and strong performance, enjoys great popularity.
%The algorithm selects hyperparameter configurations at random and uses successive halving~\citep{Jamieson2016} with different settings to early-stop less promising training runs.
%Several improvements have been proposed with the aim to replace the random sampling of hyperparameter configurations with a more guided approach.
%Among those, the most notable ones are Bayesian optimization and differential evolution~\citep{Awad2021}.
Hyperband~\citep{Li2017} is a bandits-based multi-fidelity method for hyperparameter optimization, that due to its simplicity and strong performance, enjoys great popularity.
The algorithm selects hyperparameter configurations at random and uses successive halving~\citep{Jamieson2016} with different settings to early-stop less promising training runs. 
Several improvements have been proposed to Hyperband with the aim to replace the random sampling of hyperparameter configurations with a more guided approach~\citep{Bertrand2017,Wang2018,Wistuba2017}.
BOHB~\citep{Falkner2018} uses TPE~\citep{Bergstra2011} and builds a surrogate model for every fidelity adhering to a fixed-fidelity selection scheme.
DEHB~\citep{Awad2021} samples candidates using differential evolution which handles discrete and large hyperparameter search spaces better than BOHB.

%Among those, the most notable ones are Bayesian optimization and differential evolution.
%From the domain of Bayesian optimization, BOHB uses TPE~\citep{Bergstra2011} and builds a surrogate model for every fidelity adhering to a fixed-fidelity selection scheme,  Lastly, from the domain of differential evolution, DEHB builds upon BOHB by incorporating differential evolution, thus, handling discrete and large hyperparameter search spaces better compared to BOHB.

\paragraph*{Deep Kernel Learning with Bayesian Optimization.}
We are among the first to use deep kernel learning with Bayesian optimization and to the best of our knowledge the first to use it for multi-fidelity Bayesian optimization.
\cite{Rai2016} consider the use of a deep kernel instead of a manually designed kernel in the context of standard Bayesian optimization, but, limit their experimentation to synthetic data and do not consider its use for hyperparameter optimization.
\cite{Perrone2018,Wistuba2021} use a pre-trained deep kernel to warm start Bayesian optimization with meta-data from previous optimizations.
These approaches are multi-task or transfer learning methods that require the availability of meta-data from related tasks.

%Our aim is to improve upon BOHB by developing a multi-fidelity Bayesian optimization approach that is not limited to the Hyperband bracket policy of selecting and discarding hyperparameter configurations.
%Furthermore, we use a deep kernel that allows for flexible kernel learning and overcomes the problem of manually engineering kernels.
%Finally, we propose the first surrogate model for Bayesian optimization method that explicitly takes the learning curve as an input.

In contrast to prior work, we propose the first deep kernel GP for multi-fidelity HPO that is able to capture the learning dynamics across fidelities/budgets, combined with an acquisition function that is tailored for the gray-box setup. Furthermore, our work represents an important step towards scaling HPO for Deep Learning (DL), by demonstrating a statistically significant reduction in terms of HPO time on a series of DL network architectures and a large set of diverse datasets.

==> Text/4_preliminaries.tex <==
\section{Preliminaries}
%In this section we briefly introduce the black-box and gray-box optimization problems in the context of hyperparameter optimization as well as provide an introduction to Gaussian Processes and Bayesian optimization.

\comment{
\paragraph{Black-Box Optimization.}
As mentioned earlier, the problem of optimizing hyperparameters can be modeled as a black-box optimization problem.
The objective is to maximize the response function $f:\confspace\rightarrow\mathbb{R}$ that returns the validation score for training a machine learning model with a hyperparameter configuration $\conf\in\confspace$.
In practice, this observation is noisy such that we observe in fact $y_i=f(\conf_i)+\varepsilon$ where $\varepsilon\sim\mathcal{N}(0,\sigma_n^2)$.
}
\paragraph{Gray-Box Optimization.}
Since many machine learning algorithms allow to measure at various fidelities, a relaxation of the black-box to the gray-box optimization problem is in many cases logical and allows for significantly faster optimization.
The gray-box setting allows us to query configurations with a budget smaller than the maximum budget $B$.
Thus, we can query from the response function $f:\confspace\times\mathbb{N}\rightarrow\mathbb{R}$ where $f_{i,j}=f(\conf_i, j)$ is the response after spending a budget of $j$ on configuration $\conf_i$.
As before, these observations are noisy and we observe $y_{i,j}=f(\conf_i,j)+\varepsilon_j$ where $\varepsilon_j\sim\mathcal{N}(0,\sigma_{j,n}^2)$.
Please note, we assume that the budget required to query $f_{i,j+b}$ after querying $f_{i,j}$ is only $b$.
While this is not necessarily the case for all problems, the models we consider are learned incrementally.
Furthermore, we are able to make use of the learning curve $\mathbf{Y}_{i,j-1}=(y_{i,1},\ldots,y_{i,j-1})$ when predicting $f_{i,j}$.

\comment{
\paragraph{Bayesian Optimization (BO).}
BO is a general framework for solving black-box optimization problems and is very popular for optimizing hyperparameters.
It has two ingredients, i.e. a surrogate model and an acquisition function.
The surrogate is a probabilistic model which approximates the black-box function using the available information of function evaluations.
The acquisition function returns the expected utility for a configuration given the surrogate model's prediction.
The BO framework executes the following steps sequentially.
First, the surrogate model is trained on the available information about the black-box function, denoted as the history of evaluations $\mathcal{D}$.
Then, the configuration with the highest expected utility $\conf_i$ is evaluated and $y_i$ is observed.
The tuple $(\conf_i,y_i)$ is added to $\mathcal{D}$ and the process is repeated until the HPO budget is exhausted.
A common choice for the surrogate model are Gaussian Processes~\citep{Rasmussen2006}, a popular choice for the acquisition function is expected improvement~\citep{Jones1998_Efficient}.
}

\paragraph{Gaussian Processes (GP).} GPs are probabilistic machine learning models.
Given a training data set $\mathcal{D}=\{(\conf_i,y_i)|i= 1,\ldots,n\}$ with $n$ data points, the Gaussian Process assumption is that $y_{i}$ is a random variable and the joint distribution of all $y_{i}$ is assumed to be multivariate Gaussian distributed as:
\begin{equation}
\mathbf{y}\sim\mathcal{N}\left(m\left(\Conf\right),\kernel\left(\Conf,\Conf\right)\right)\enspace \label{eq:definition-joint-likelihood}
\end{equation}
Furthermore, $\mathbf{f}_{*}$ for test instances $\conf_{*}$ are jointly Gaussian with $\mathbf{y}$ as:
\begin{equation}
\left[\begin{array}{c}
\mathbf{y}\\
\mathbf{f}_{*}
\end{array}\right]\sim\mathcal{N}\left(m\left(\Conf,\conf_{*}\right),\left(\begin{array}{cc}
\mathbf{K}_{n} & \mathbf{K}_{*}\\
\mathbf{K}_{*}^{T} & \mathbf{K}_{**}
\end{array}\right)\right)\enspace.
\end{equation}
The mean function $m$ is often set to $\mathbf{0}$ and its covariance function $\kernel$ depends on parameters $\boldsymbol{\theta}$.
For notational convenience, we use:
\begin{align}
\mathbf{K}_{n} &= \kernel\left(\Conf,\Conf|\boldsymbol{\theta}\right)+\sigma_{n}^{2}\mathbf{I},\\ 
\mathbf{K}_{*} &=  \kernel\left(\Conf,\Conf_{*}|\boldsymbol{\theta}\right), \nonumber \\
\mathbf{K}_{**} &=  \kernel\left(\Conf_{*},\Conf_{*}|\boldsymbol{\theta}\right) \nonumber
\end{align}
to define the kernel matrix.
We can derive the posterior predictive distribution with mean and covariance as follows:
\begin{align}
\label{eq:gp-mean-cov}
\mathbb{E}\left[\mathbf{f}_{*}|\Conf,\mathbf{y},\Conf_*\right] &= \mathbf{K}_{*}^{T}\mathbf{K}_{n}^{-1}\mathbf{y},\\ \nonumber
\text{cov}\left[\mathbf{f}_{*}|\Conf,\Conf_*\right] &= \mathbf{K}_{**}-\mathbf{K}_{*}^{T}\mathbf{K}_{n}^{-1}\mathbf{K}_{*}
\end{align}

Often, the kernel function is manually engineered, one popular example is the squared exponential kernel.
However, in this work, we make use of the idea of deep kernel learning~\citep{Wilson2016}.
The idea is to model the kernel as a neural network $\varphi$ and learn the best kernel transformation as:
\begin{equation}
    \kernel_{\text{deep}}(\conf,\conf'|\boldsymbol{\theta},\mathbf{w})=\kernel(\varphi(\conf,\mathbf{w}),\varphi(\conf',\mathbf{w})|\boldsymbol{\theta}).
\end{equation}
As we will see later, this allows us to use convolutional operations as part of our kernel.

==> Text/7_old_results.tex <==
\section{Results} 
%\subsection{Feedforward Neural Networks}

\paragraph{MLP Search Space} In our first experiment, we evaluate the various methods on how well they optimize neural networks for tabular datasets.
For this purpose, we use the LCBench learning curve benchmark~\citep{Zimmer2021}.
This benchmark contains learning curves for 35 different datasets where 2,000 neural networks per dataset are trained for 50 epochs with Auto-PyTorch.
The objective is to optimize seven different hyperparameters of funnel-shaped neural networks, i.e., batch size, learning rate, momentum, weight decay, dropout, number of layers, and maximum number of units per layer.
We show the aggregated results in Figure~\ref{fig:aggregated_results_lcbench}. Here we aggregate the normalized wallclock time by dividing the actual wallclock time of baselines by the total wallclock time of our method \algabbr{} including the overhead incurred by fitting the deep GP. In that manner, we can aggregate wallclock times across datasets.
However, all the results for each individual dataset are reported in the Appendix (Figure \ref{fig:results_per_dataset1} and \ref{fig:results_per_dataset2}).
Furthermore, we use a critical difference diagram to report the pairwise statistical difference between all methods (Figure~\ref{fig:lcbench-cr}).
Horizontal lines indicate groups of methods that are not significantly different from each other.
As suggested in the work of \cite{Demsar2006}, we use the Friedman test to reject the null hypothesis followed by a pairwise posthoc analysis based on the Wilcoxon signed-rank test ($\alpha=0.05$). While all gray-box methods have a very similar performance in the very beginning, \algabbr{} quickly outperforms its competitors with respect to both evaluation metrics with statistical significance.
%Notably, the average rank converges towards 1, indicating that \algabbr{} is performing the best on almost every dataset.
On this task, both BOHB and DEHB are significantly better than Hyperband but there is no clear winner among these two methods.
%Without a doubt, random search is providing the worst results as expected, since, it is not early-stopping any candidate configuration.


\begin{figure}[t]
  \centering
    \includegraphics[width=0.49\columnwidth]{fig/lcbench/cr_499.pdf}
    \includegraphics[width=0.49\columnwidth]{fig/lcbench/cr_999.pdf}
    \includegraphics[width=0.49\columnwidth]{fig/taskset/cr_499.pdf}
    \includegraphics[width=0.49\columnwidth]{fig/taskset/cr_999.pdf}

  \caption{Critical difference diagram for LCBench for results corresponding to the time \algabbr{} took to complete 200, 600 and 1,000 epochs. \algabbr{}'s improvement is statistically significant.}
  \label{fig:lcbench-cr}
\end{figure}

\begin{figure*}[t]
  \centering
    \includegraphics[width=0.29\textwidth]{fig/lcbench/overhead_aggregate_results.pdf}
    \includegraphics[width=0.4\textwidth]{fig/nasbench201/overhead_ImageNet16-120_main.pdf}
    \hfill
    \begin{minipage}{0.28\textwidth}
    \vspace{-4cm}
    \includegraphics[width=\textwidth]{fig/lcbench/overhead_cr_0.50.pdf}\\
    \includegraphics[width=\textwidth]{fig/lcbench/overhead_cr_1.0.pdf}
    \end{minipage}
  \caption{TODO}
\end{figure*}

\subsection{Recurrent Neural Networks}
We continue with evaluating all methods on NLP tasks using search spaces provided in TaskSet~\citep{Metz2020}.
The objective is to optimize eight hyperparameters for a set of different recurrent neural networks (RNN) that differ in embedding size, RNN cell, and other architectural features.
The set of hyperparameters consists of optimizer-specific hyperparameters, such as the learning rate, the exponential decay rate of the first and second momentum of Adam, $\beta_1$ and $\beta_2$, and Adam's constant for numerical stability $\varepsilon$.
Furthermore, there are two hyperparameters controlling linear and exponential learning rate decays, as well as L1 and L2 regularization terms.
As before, we provide the aggregated results in the main paper (Figure~\ref{fig:aggregated_results_taskset}) and provide detailed results in the Appendix (Figure~\ref{fig:results_per_dataset_taskset}).
We show the critical difference diagram in Figure~\ref{fig:taskset-cr}.
As before, all gray-box methods have a very similar performance in the very beginning, but, \algabbr{} quickly outperforms its competitors with respect to both evaluation metrics.
The difference is significant in the first interval measured, in fact, \algabbr{} is providing the best results across all different tasks for the majority of the elapsed time.
Given enough time, BOHB is able to catch up but \algabbr{}'s improvement is still statistically significant.





\begin{figure}[t]
  \centering
    %\includegraphics[width=0.45\textwidth]{fig/ablation/lcbench/mean_regret.pdf}
    \includegraphics[width=0.7\columnwidth]{fig/ablation/nasbench201/ImageNet16-120.pdf}

  \caption{Left: Aggregated results for LCBench. Right: Results on ImageNet from NAS-Bench 201.
  Using the learning curve gives only little advantage on average for the LCBench problems.
  However, not using it significantly worsens it for the NAS-Bench 201 tasks.}
  \label{fig:ablation_main}
\end{figure}


\subsection{Convolutional Neural Networks}

Neural Architecture Search~\citep{Zoph2017} (NAS) raised a lot of interest in the deep learning community in the last few years.
Since it can be reformulated to a hyperparameter optimization problem, we can apply our method as well as many other standard hyperparameter optimization methods to it.
We refrain from comparing against specialized NAS methods, since, this is out-of-scope for our work but refer the interested reader to the comparison of \cite{Dong2020}.
To evaluate our methods in this scenario, we use NAS-Bench-201~\citep{Dong2020}.
This benchmark has precomputed about 15,600 architectures trained for 200 epochs for the image classification datasets CIFAR-10, CIFAR-100, and ImageNet.
The objective is to select for each of the six operations within the cell of the macro architecture one of five different operations.
All other hyperparameters such as learning rate and batch size are kept fix.
We report the results in Figure~\ref{fig:results_nasbench201_imagenet}, the remaining results can be found in the Appendix (Figure~\ref{fig:results_nasbench201_time}).
Initially, \algabbr{} provides better results, but, given enough time, most methods perform no longer significantly different.
We see also no difference between Hyperband and BOHB or DEHB.
A reason for this observation will be discussed in the next section.

\paragraph{On the efficiency of \algabbr{}.}

\begin{figure*}[t]
  \centering
    \includegraphics[width=0.32\textwidth]{fig/precision_lcbench.pdf}
    \includegraphics[width=0.32\textwidth]{fig/avg_regret_lcbench.pdf}
    \includegraphics[width=0.32\textwidth]{fig/promotions_lcbench.pdf}

  \caption{The efficacy of \algabbr{}. \textbf{Left:} The fraction of top-performing candidates from all candidates that were selected to be trained. \textbf{Middle:} The average regret for the configurations that were selected to be trained at a given budget. \textbf{Right:} The percentage of configurations that belong to the top 1/3 configurations at a given budget and that were in the top bottom 2/3 of the configurations at a previous budget. All of the results are from the LCBench benchmark.}
  \label{fig:dyhpo_efficiency}
\end{figure*}

In Figure~\ref{fig:dyhpo_efficiency}, we plot the precision of every method for different considered budgets, which clearly shows that \algabbr{} \textbf{effectively explores the search space and identifies promising candidates}.
The precision at an epoch $i$ is defined as the number of top 1\% candidates trained divided by the number of all candidates trained, both trained for at least $i$ epochs.
The higher the precision, the less irrelevant candidates were considered and the less computational resources were wasted.
For small budgets, the precision is low since \algabbr{} spends budget to consider a few candidates but then promising candidates are successfully identified and the precision quickly increases. On the contrary, the other methods dedicate significantly more resources to irrelevant candidates which explains why \algabbr{} finds good candidates faster.

This argument is further supported by Figure~\ref{fig:dyhpo_efficiency}, where we visualize the \textbf{average} regret of \textbf{all} the candidates trained for at least the specified number of epochs in the x-axis. In contrast to the regret plots, here we do not show the regret of the \textbf{best} configuration, but the mean regret of \textbf{all} the selected configurations. The analysis deduces a similar finding, our method \algabbr{} selects highly more qualitative hyperparameter configurations than all the baselines.

An interesting property of multi-fidelity HPO is the phenomenon of poor rank correlations among the validation performance of candidates at different budgets. In other words, a configuration that achieves a poor performance at a small budget, might perform strongly at a larger budget. For instance, a well-regularized neural network will converge slower than an un-regularized network in the early optimization epochs, but eventually performs better when converged. We analyze this phenomenon and report the respective results in Figure~\ref{fig:promotions}. In this experiment we measure the percentage of "good"  configurations at a particular budget, that were "bad" performers in at least one of the smaller budgets. We define a "good" performance at a budget B, when a configuration achieves a validation accuracy ranked among the top 1/3 compared to the validation accuracies of all the other configurations that were run until that budget B. Similarly a "bad" performance at a budget B represents a configuration whose validation accuracy belongs to the bottom 2/3 of all configurations run at that budget B. 

In Figure~\ref{fig:promotions} we analyze the percentage of "good" configurations at each budget denoted by the x-axis, that were "bad" performers in at least one of the lower budgets. Such a metric is a proxy for the degree of the promotion of "bad" configurations towards higher budgets. We present the analysis for all the competing methods of our experimental protocol from Section~\ref{sec:experiments}. We have additionally included the ground-truth line annotated as "Baseline", which represents the fraction of past poor performers among all the feasible configurations in the search space. In contrast, the respective methods compute the fraction of promotions only among the configurations that those methods have considered (i.e. selected within their HPO trials) until the budget indicated by the x-axis. We see that in all the search spaces LCBench, TaskSet and NASBench-201 there is a high degree of "good" configurations that were "bad" at a previous budget, with fractions of the ground-truth "Baseline" varying from ca. 40\% in LCBench, up to ca. 70\% in the NASBench-201 datasets.  

On the other hand, the analysis demonstrates that our method \algabbr{} has promoted more "good" configurations that were "bad" in a lower budget, compared to all the rival methods. In particular, ca. 80\% of selected configurations at the datasets from the LCBench benchmark were "bad" performers at a lower budget, while in the case of NASBench-201 this fraction approaches the level of 95\%.

\subsection{Ablation Study}
One of the main differences between \algabbr{} and similar methods such as the work by \cite{Kandasamy2017}, is that the learning curve is an input to the kernel function.
For this reason, we investigate the impact of this design choice.
We consider a variation of \algabbr{}, \algabbr{} w/o LC, which is identical to its counterpart, and the only difference is that the learning curve is not part of the input.
We report the results in Figure~\ref{fig:ablation_main} and refer to the Appendix for additional results (Figure~\ref{fig:results_nasbench201_ablation}).
One of the striking observations is that the learning curve has only a small impact for LCBench in contrast to NAS-Bench-201 where it is significant.
Our hypothesis is that for LCBench the hyperparameter representation is a valuable feature such that the additional use of the learning curve (which in fact is already implicitly considered by the Gaussian Process) is not required.
For NAS-Bench 201, however, the architecture representation is poor and does not allow for good predictions on its own.
This hypothesis aligns well with our previous experiments, where BOHB did better on LCBench compared to Hyperband whereas we have not seen any difference on NAS-Bench 201.
As a reminder, BOHB is a variation of Hyperband that considers the hyperparameter representation to sample candidates.

We conclude, that the additional use of an explicit learning curve representation might not lead to a strong improvement in every scenario, however, it also does not seem to deteriorate it.
Furthermore, there are cases where the explicit consideration leads to significantly better results.
